How close are we to understanding image-based saliency?

Within the set of the many complex factors driving gaze placement, the properities of an image that are associated with fixations under free viewing conditions have been studied extensively. There is a general impression that the field is close to understanding this particular association. Here we frame saliency models probabilistically as point processes, allowing the calculation of log-likelihoods and bringing saliency evaluation into the domain of information. We compared the information gain of state-of-the-art models to a gold standard and find that only one third of the explainable spatial information is captured. We additionally provide a principled method to show where and how models fail to capture information in the fixations. Thus, contrary to previous assertions, purely spatial saliency remains a significant challenge.

==> figures/auc_examples.tex <==

\newcommand{\contrastHighFixHighSmapLoglikelihood}{2.93}
\newcommand{\contrastHighFixLowSmapLoglikelihood}{0.08}
\newcommand{\contrastLowFixHighSmapLoglikelihood}{-1.82}
\newcommand{\contrastLowFixLowSmapLoglikelihood}{0.00}

\newcommand{\contrastHighFixHighSmapAUC}{86}
\newcommand{\contrastHighFixLowSmapAUC}{86}
\newcommand{\contrastLowFixHighSmapAUC}{50}
\newcommand{\contrastLowFixLowSmapAUC}{50}

\newcommand{\orderingGoodLoglikelihood}{2.23}
\newcommand{\orderingBadLoglikelihood}{0.77}

\newcommand{\orderingGoodAUC}{81}
\newcommand{\orderingBadAUC}{85}



==> figures/ig_colors.tex <==
\definecolor{colordensity}{rgb}{0.19921875, 0.625, 0.171875}
\definecolor{colorsaliency}{rgb}{0.6953125, 0.87109375, 0.5390625}
\definecolor{colorig}{rgb}{0.12109375, 0.46875, 0.703125}
\definecolor{colorigdiff}{rgb}{0.6484375, 0.8046875, 0.88671875}


==> figures/information_gains_Judd.tex <==
\filldraw (2.75628735815, 51.7778077114) circle (1pt);
\filldraw (2.24298312186, 51.9345279198) circle (1pt);
\filldraw (2.97801211785, 53.3270188878) circle (1pt);
\filldraw (2.34572990786, 47.5288515323) circle (1pt);
\filldraw (2.61244411197, 36.6802400069) circle (1pt);
\filldraw (2.58626052495, 32.9004325156) circle (1pt);
\filldraw (2.46729941717, 59.7789744244) circle (1pt);
\filldraw (2.30747631695, 41.6777382862) circle (1pt);
\filldraw (3.33078763402, 33.6166200558) circle (1pt);
\filldraw (2.91484561608, 44.0258370413) circle (1pt);
\filldraw (2.60360118347, 21.4792056624) circle (1pt);
\filldraw (2.66507773942, 54.7511791629) circle (1pt);
\filldraw (2.31997095442, 60.8323745741) circle (1pt);
\filldraw (3.65515491734, 44.3581322062) circle (1pt);
\filldraw (3.0329520141, 52.9031563658) circle (1pt);
\filldraw (2.95968348844, 1.18273322544) circle (1pt);
\filldraw (2.95155992666, 58.3111200576) circle (1pt);
\filldraw (3.22235926758, 43.0278198769) circle (1pt);
\filldraw (2.46373672668, 54.8962643601) circle (1pt);
\filldraw (2.66197679004, 50.3248274243) circle (1pt);
\filldraw (2.78988300487, 34.0752975391) circle (1pt);
\filldraw (3.07605779985, 29.337201874) circle (1pt);
\filldraw (2.41016676761, 6.08408214439) circle (1pt);
\filldraw (2.51526082509, 53.6352449875) circle (1pt);
\filldraw (3.81813052482, 84.1023629582) circle (1pt);
\filldraw (3.30915494738, 70.515231397) circle (1pt);
\filldraw (2.33948031515, 48.3213268203) circle (1pt);
\filldraw (2.8048642717, 52.2556897449) circle (1pt);
\filldraw (2.64395860481, 50.8854858845) circle (1pt);
\filldraw (3.63572265949, 68.6278862538) circle (1pt);
\filldraw (2.457339633, 20.8192945585) circle (1pt);
\filldraw (2.92782906242, 49.0443829995) circle (1pt);
\filldraw (3.15958971312, 34.7170484911) circle (1pt);
\filldraw (2.53905930651, 39.1499429608) circle (1pt);
\filldraw (2.67685357278, 44.942209554) circle (1pt);
\filldraw (3.17318514919, 45.084277923) circle (1pt);
\filldraw (1.90385760345, 32.5587046248) circle (1pt);
\filldraw (3.46555938588, 71.5309829074) circle (1pt);
\filldraw (2.57801224683, 40.5713411677) circle (1pt);
\filldraw (2.2767703124, 38.3737490743) circle (1pt);
\filldraw (3.12969729221, 27.6739024166) circle (1pt);
\filldraw (2.95895927482, 49.8354636793) circle (1pt);
\filldraw (2.70467463589, 46.0120149144) circle (1pt);
\filldraw (2.80848882487, 38.5616884201) circle (1pt);
\filldraw (3.04135161212, 47.8970304601) circle (1pt);
\filldraw (2.97251555438, 39.1068879402) circle (1pt);
\filldraw (2.88106941369, 34.8518383257) circle (1pt);
\filldraw (2.24093688711, 38.6808894954) circle (1pt);
\filldraw (2.65369274586, 48.8871838261) circle (1pt);
\filldraw (2.80917533892, 46.9629391868) circle (1pt);
\filldraw (2.85036608977, 41.2275048429) circle (1pt);
\filldraw (2.45270722533, 35.2824077622) circle (1pt);
\filldraw (3.09639755938, 67.4081426761) circle (1pt);
\filldraw (2.88591605328, 42.4626698155) circle (1pt);
\filldraw (2.60982746578, 30.8699037146) circle (1pt);
\filldraw (2.21117352229, 33.0949682823) circle (1pt);
\filldraw (2.09361467566, 40.2387197215) circle (1pt);
\filldraw (2.53027408135, 47.6351682076) circle (1pt);
\filldraw (2.55499748005, 53.6971241993) circle (1pt);
\filldraw (2.95135185707, 53.5530991857) circle (1pt);
\filldraw (2.7834354129, 61.1711489813) circle (1pt);
\filldraw (2.4971459385, 54.4813802597) circle (1pt);
\filldraw (2.56999572106, 58.9129611378) circle (1pt);
\filldraw (2.87800355161, 22.5800219804) circle (1pt);
\filldraw (3.47940927804, 55.301861853) circle (1pt);
\filldraw (2.96895017484, 54.3579054412) circle (1pt);
\filldraw (2.41327908521, 43.5329743112) circle (1pt);
\filldraw (2.56496598565, 36.3995042651) circle (1pt);
\filldraw (2.64653803204, 61.3114627673) circle (1pt);
\filldraw (3.11256125497, 49.6928068085) circle (1pt);
\filldraw (2.4912851486, 45.3516144113) circle (1pt);
\filldraw (2.85631184337, 51.2006319053) circle (1pt);
\filldraw (2.92914629726, 39.2286198175) circle (1pt);
\filldraw (2.79746594029, 60.5833186606) circle (1pt);
\filldraw (2.48143731709, 31.4268888869) circle (1pt);
\filldraw (3.9494449262, 58.138630814) circle (1pt);
\filldraw (3.0749608549, 56.1774300378) circle (1pt);
\filldraw (3.03872454688, 56.4048563975) circle (1pt);
\filldraw (3.35075873339, 48.5645565163) circle (1pt);
\filldraw (3.21927412194, 31.3117516443) circle (1pt);
\filldraw (2.70169877705, 57.1429216395) circle (1pt);
\filldraw (2.62709222423, 42.0062561991) circle (1pt);
\filldraw (2.1453917887, 43.850008421) circle (1pt);
\filldraw (2.23419042313, 48.6242165085) circle (1pt);
\filldraw (3.34322780157, 39.4575420454) circle (1pt);
\filldraw (3.72488817418, 55.7534492897) circle (1pt);
\filldraw (3.04448850223, 37.112477003) circle (1pt);
\filldraw (3.39107048598, 19.025279193) circle (1pt);
\filldraw (2.60316719083, 64.5335340152) circle (1pt);
\filldraw (3.1521985385, 45.6850880831) circle (1pt);
\filldraw (2.40548775918, 51.8225016792) circle (1pt);
\filldraw (2.34886881669, 50.9544424636) circle (1pt);
\filldraw (2.69636621937, 42.5726668782) circle (1pt);
\filldraw (2.47722364939, 28.0982288251) circle (1pt);
\filldraw (2.26843358119, 24.1124382609) circle (1pt);
\filldraw (2.48210412197, 57.3202796027) circle (1pt);
\filldraw (2.81407573955, 33.7183921122) circle (1pt);
\filldraw (3.33659759686, 63.4312365195) circle (1pt);
\filldraw (3.49161934471, 59.2902785122) circle (1pt);
\filldraw (2.84128625467, 20.2787038053) circle (1pt);
\filldraw (2.18652098541, 42.9635293201) circle (1pt);
\filldraw (2.28160163129, 24.0994843579) circle (1pt);
\filldraw (2.69800434151, 20.3806017694) circle (1pt);
\filldraw (3.19288271646, 48.5719687105) circle (1pt);
\filldraw (2.76297904171, 39.2731277165) circle (1pt);
\filldraw (2.68062227435, 50.7158139508) circle (1pt);
\filldraw (2.82153332929, 45.6071740306) circle (1pt);
\filldraw (3.11659150638, 17.5049571484) circle (1pt);
\filldraw (3.13468662555, 47.5831413983) circle (1pt);
\filldraw (3.54607667145, 51.3803306805) circle (1pt);
\filldraw (2.29647128477, 28.7711855957) circle (1pt);
\filldraw (2.38228508563, 44.4633605788) circle (1pt);
\filldraw (3.15435965733, 33.0185569999) circle (1pt);
\filldraw (2.83774912265, 50.6339479796) circle (1pt);
\filldraw (2.81871652392, 52.1147394385) circle (1pt);
\filldraw (2.82441855463, 60.8354599637) circle (1pt);
\filldraw (2.78150939745, 5.77170961451) circle (1pt);
\filldraw (3.90084227816, 58.736770005) circle (1pt);
\filldraw (2.76323718248, 23.6566978896) circle (1pt);
\filldraw (3.06804589243, 46.0931565326) circle (1pt);
\filldraw (3.30631134059, 27.8762717198) circle (1pt);
\filldraw (2.98492162199, 31.6470050827) circle (1pt);
\filldraw (2.75285773065, 53.37876822) circle (1pt);
\filldraw (2.68918909611, 51.3781383754) circle (1pt);
\filldraw (4.09781856656, 42.1239032523) circle (1pt);
\filldraw (2.6180121029, 37.7061193162) circle (1pt);
\filldraw (3.77904424789, 46.9769596376) circle (1pt);
\filldraw (2.95777341877, 50.9911110422) circle (1pt);
\filldraw (2.38934020862, 26.9326411724) circle (1pt);
\filldraw (3.17122607663, 45.4653284143) circle (1pt);
\filldraw (4.17575852741, 45.6451184543) circle (1pt);
\filldraw (2.49199406207, 24.2292918314) circle (1pt);
\filldraw (2.92435861971, 46.1658605973) circle (1pt);
\filldraw (3.10809272865, 34.7755814149) circle (1pt);
\filldraw (2.86020579265, 60.7200686357) circle (1pt);
\filldraw (3.26637437632, 37.663769776) circle (1pt);
\filldraw (3.2133085336, 23.2297528507) circle (1pt);
\filldraw (2.36901958624, 50.1686725666) circle (1pt);
\filldraw (2.92052275717, 52.5769909299) circle (1pt);
\filldraw (2.77900464806, 30.5733401403) circle (1pt);
\filldraw (2.29729335467, 39.1151571888) circle (1pt);
\filldraw (2.76635762228, 13.9116377156) circle (1pt);
\filldraw (3.76452829744, 69.9965118366) circle (1pt);
\filldraw (3.05335508826, 40.1606421726) circle (1pt);
\filldraw (3.22181726739, 49.5492072345) circle (1pt);
\filldraw (2.95637804486, 45.7062340876) circle (1pt);
\filldraw (2.61274754154, 56.6892688004) circle (1pt);
\filldraw (2.33694479808, 41.1136922606) circle (1pt);
\filldraw (3.50821376546, 57.4305396916) circle (1pt);
\filldraw (2.324765685, 46.033426571) circle (1pt);
\filldraw (2.5021883186, 50.5323938577) circle (1pt);
\filldraw (3.08781745451, 54.8722063944) circle (1pt);
\filldraw (2.43583394796, 61.3353797786) circle (1pt);
\filldraw (3.08916204695, 35.8934333506) circle (1pt);
\filldraw (2.55755129544, 52.1497972463) circle (1pt);
\filldraw (2.74417990566, 63.3683109156) circle (1pt);
\filldraw (2.44202478994, 29.5656872194) circle (1pt);
\filldraw (3.1795299594, 56.0184551476) circle (1pt);
\filldraw (2.32936807493, 52.2449028532) circle (1pt);
\filldraw (3.204625918, 55.00603313) circle (1pt);
\filldraw (3.24176822975, 24.8739584051) circle (1pt);
\filldraw (2.77567353362, 4.99458508444) circle (1pt);
\filldraw (2.46424967258, 14.3599224289) circle (1pt);
\filldraw (2.57849895356, 65.1988504923) circle (1pt);
\filldraw (3.53481742706, 53.8118454592) circle (1pt);
\filldraw (2.42944163452, -1.60217467825) circle (1pt);
\filldraw (2.35113463883, 49.1545969211) circle (1pt);
\filldraw (3.86309982107, 28.0645602087) circle (1pt);
\filldraw (3.71369348777, 57.4091157094) circle (1pt);
\filldraw (2.63934227042, 61.4444744496) circle (1pt);
\filldraw (2.702170052, -15.1975209832) circle (1pt);
\filldraw (2.76545639724, 47.9330703361) circle (1pt);
\filldraw (3.33962827315, 30.4712204137) circle (1pt);
\filldraw (2.92544900927, 68.8117257136) circle (1pt);
\filldraw (2.39583582869, 30.2753923096) circle (1pt);
\filldraw (2.74174749, 65.5986550941) circle (1pt);
\filldraw (2.69296637046, 51.2472126592) circle (1pt);
\filldraw (3.0855296822, 49.6578120618) circle (1pt);
\filldraw (2.11591504049, 30.8967087536) circle (1pt);
\filldraw (3.14852808913, 50.2686973668) circle (1pt);
\filldraw (2.79445584341, 58.2065389475) circle (1pt);
\filldraw (2.79599905623, 61.6125406359) circle (1pt);
\filldraw (1.85726770026, 52.1028897823) circle (1pt);
\filldraw (2.69981616984, 38.919138532) circle (1pt);
\filldraw (2.25890958952, 9.15035106925) circle (1pt);
\filldraw (2.2669950975, 29.6202320985) circle (1pt);
\filldraw (3.15540188569, 36.1017918764) circle (1pt);
\filldraw (2.50188485039, 31.1148455642) circle (1pt);
\filldraw (3.44037931922, 43.4989033514) circle (1pt);
\filldraw (2.92390830976, 42.9899387108) circle (1pt);
\filldraw (3.11674458299, 37.1623574899) circle (1pt);
\filldraw (2.36098134693, 39.1753352415) circle (1pt);
\filldraw (3.39673105057, 57.0565391307) circle (1pt);
\filldraw (2.79249615531, 54.9551451575) circle (1pt);
\filldraw (2.63144322244, 23.9138946701) circle (1pt);
\filldraw (2.79443179581, 24.1598960904) circle (1pt);
\filldraw (2.56705273233, 42.3431366818) circle (1pt);
\filldraw (2.6916933733, 40.9631134711) circle (1pt);
\filldraw (2.86363739968, 61.3656836345) circle (1pt);
\filldraw (2.80006180504, 40.1269259319) circle (1pt);
\filldraw (3.04818473348, 37.1070854196) circle (1pt);
\filldraw (2.77699908715, 59.0964275479) circle (1pt);
\filldraw (3.8015607397, 25.8048540135) circle (1pt);
\filldraw (2.48281194638, 21.4883539909) circle (1pt);
\filldraw (2.65659881831, 52.7375639101) circle (1pt);
\filldraw (2.30168222691, 45.9906515127) circle (1pt);
\filldraw (2.43436823546, 36.23687731) circle (1pt);
\filldraw (2.25662724973, 30.6401354568) circle (1pt);
\filldraw (2.57887876166, 28.6922349634) circle (1pt);
\filldraw (2.71654738539, 19.6453784618) circle (1pt);
\filldraw (3.06319590806, 47.1353698364) circle (1pt);
\filldraw (2.19869388505, 24.5126365799) circle (1pt);
\filldraw (3.55555396812, 68.1281850447) circle (1pt);
\filldraw (3.11704792023, 62.3193150891) circle (1pt);
\filldraw (3.2352143723, 51.0777280516) circle (1pt);
\filldraw (2.15334701869, 40.0365517736) circle (1pt);
\filldraw (2.79650190679, 58.4891789986) circle (1pt);
\filldraw (2.76732034248, 42.9495912199) circle (1pt);
\filldraw (2.86662875205, 55.3246579414) circle (1pt);
\filldraw (3.09855643238, 22.9615104155) circle (1pt);
\filldraw (3.35362812086, 42.8841104332) circle (1pt);
\filldraw (3.30158312847, 54.6879105053) circle (1pt);
\filldraw (2.41234898302, 59.539540513) circle (1pt);
\filldraw (3.04933414907, 36.5318913155) circle (1pt);
\filldraw (3.1514403271, 36.0581288968) circle (1pt);
\filldraw (2.49876679641, 25.0258207103) circle (1pt);
\filldraw (3.04317580738, 15.2064255262) circle (1pt);
\filldraw (3.98942212466, 56.6146473035) circle (1pt);
\filldraw (2.67003144792, -38.2016046207) circle (1pt);
\filldraw (2.57219326496, 43.3447993386) circle (1pt);
\filldraw (3.10064490939, 47.0680810651) circle (1pt);
\filldraw (2.89130020701, 44.3481413838) circle (1pt);
\filldraw (4.21482792059, 63.6749275978) circle (1pt);
\filldraw (2.98808396391, 56.1491502142) circle (1pt);
\filldraw (2.8667541359, 43.7989241969) circle (1pt);
\filldraw (2.38897425327, 51.8091993789) circle (1pt);
\filldraw (3.55701301457, 65.9712909132) circle (1pt);
\filldraw (2.90372417752, 28.2626916806) circle (1pt);
\filldraw (3.24352323956, 45.3958213531) circle (1pt);
\filldraw (3.0794856707, 42.4876650171) circle (1pt);
\filldraw (2.90682756203, 39.2761799412) circle (1pt);
\filldraw (2.6584328992, 42.50952501) circle (1pt);
\filldraw (3.02438462868, 63.8058035365) circle (1pt);
\filldraw (2.29298655025, 36.62654631) circle (1pt);
\filldraw (2.68213757045, 23.5176464008) circle (1pt);
\filldraw (3.45742828884, 48.6674363595) circle (1pt);
\filldraw (3.4943148838, 5.69646149549) circle (1pt);
\filldraw (3.41681721143, 42.811299521) circle (1pt);
\filldraw (2.51380355887, 50.9444309605) circle (1pt);
\filldraw (2.84805957288, 53.2655864637) circle (1pt);
\filldraw (1.9923127202, 49.1866597379) circle (1pt);
\filldraw (2.81408542949, 34.2609165091) circle (1pt);
\filldraw (2.89517648226, 25.5385261576) circle (1pt);
\filldraw (3.07466586169, 67.6197070729) circle (1pt);
\filldraw (2.53002213323, 44.2306390302) circle (1pt);
\filldraw (2.7127547372, 50.4998405144) circle (1pt);
\filldraw (2.53320257013, 20.8190790895) circle (1pt);
\filldraw (2.24148953834, -9.03829213326) circle (1pt);
\filldraw (2.31539909856, 42.7859668141) circle (1pt);
\filldraw (2.2689990907, 35.5201234688) circle (1pt);
\filldraw (2.63574670666, 55.009660465) circle (1pt);
\filldraw (3.46587805049, 67.6626898858) circle (1pt);
\filldraw (3.00742348204, 32.2870190042) circle (1pt);
\filldraw (3.69600466214, 63.6290229318) circle (1pt);
\filldraw (2.8779700098, 15.0901834556) circle (1pt);
\filldraw (2.48161775132, 53.8471888823) circle (1pt);
\filldraw (2.13691668521, 47.1510754199) circle (1pt);
\filldraw (1.85360670891, 1.39319697026) circle (1pt);
\filldraw (3.02445201106, 54.1627661176) circle (1pt);
\filldraw (2.84908920095, 28.0833760851) circle (1pt);
\filldraw (3.54775233476, 20.9237117271) circle (1pt);
\filldraw (3.71148900205, 43.3220131388) circle (1pt);
\filldraw (2.92452587279, 69.7598789247) circle (1pt);
\filldraw (2.67757696734, -0.630042696579) circle (1pt);
\filldraw (2.04051854342, 40.8525132262) circle (1pt);
\filldraw (3.231479136, 68.2313975678) circle (1pt);
\filldraw (2.68650596684, 43.1258937153) circle (1pt);
\filldraw (3.29891944332, 63.4146059814) circle (1pt);
\filldraw (2.79971815649, 20.2455629768) circle (1pt);
\filldraw (2.96533058946, 46.9477287802) circle (1pt);
\filldraw (2.54957640485, 49.482089502) circle (1pt);
\filldraw (2.70499912965, 55.5638414958) circle (1pt);
\filldraw (2.50093315963, 27.2236129204) circle (1pt);
\filldraw (3.06235061038, 60.5887330348) circle (1pt);
\filldraw (1.96131531408, 40.480448114) circle (1pt);
\filldraw (2.79866322861, -21.3906081122) circle (1pt);
\filldraw (2.63714362481, 18.4815674149) circle (1pt);
\filldraw (3.28693598115, 37.5476373251) circle (1pt);
\filldraw (3.90878239968, 59.7737845676) circle (1pt);
\filldraw (2.76491782628, 42.2719693947) circle (1pt);
\filldraw (2.50879054867, 42.5304976422) circle (1pt);
\filldraw (2.31029140575, 54.0187247885) circle (1pt);
\filldraw (3.20079429964, 44.4956190337) circle (1pt);
\filldraw (3.57633033988, 50.5102952834) circle (1pt);
\filldraw (2.29268959165, 37.7444022889) circle (1pt);
\filldraw (2.94967417629, 52.197844384) circle (1pt);
\filldraw (3.00894124182, 32.7284340226) circle (1pt);
\filldraw (2.73384957096, 29.0318333575) circle (1pt);
\filldraw (1.97096492885, 27.0894404925) circle (1pt);
\filldraw (3.01912063727, 53.9583888333) circle (1pt);
\filldraw (2.33943210156, 61.8518228136) circle (1pt);
\filldraw (2.83421691085, 25.2247218128) circle (1pt);
\filldraw (2.37405008767, 17.3517332792) circle (1pt);
\filldraw (3.84481353269, 61.5239120388) circle (1pt);
\filldraw (3.24120424267, 50.6388051588) circle (1pt);
\filldraw (2.61527779345, 23.3705946918) circle (1pt);
\filldraw (2.61885074379, 51.0212834268) circle (1pt);
\filldraw (2.83347546389, 57.6007391895) circle (1pt);
\filldraw (2.59875621755, 43.7406486778) circle (1pt);
\filldraw (2.41199812649, 54.236021244) circle (1pt);
\filldraw (2.27786707343, 27.5874466855) circle (1pt);
\filldraw (2.75118687756, 52.9046203057) circle (1pt);
\filldraw (2.35543509058, 48.2090891376) circle (1pt);
\filldraw (3.23648097861, 65.5535512155) circle (1pt);
\filldraw (2.40787106924, 58.8758204983) circle (1pt);
\filldraw (2.06017594745, 37.2626522912) circle (1pt);
\filldraw (3.62416199961, 48.6560103766) circle (1pt);
\filldraw (2.9873891576, 57.4737883817) circle (1pt);
\filldraw (2.29672095846, 40.8282404556) circle (1pt);
\filldraw (2.14627504496, 39.7355921944) circle (1pt);
\filldraw (3.39428630244, 16.1498946879) circle (1pt);
\filldraw (3.28408801105, 59.7802900813) circle (1pt);
\filldraw (4.02850252866, 56.1808536085) circle (1pt);
\filldraw (2.66156506891, -7.32005452297) circle (1pt);
\filldraw (3.69840764902, 45.4213876458) circle (1pt);
\filldraw (2.94640229489, 54.1147962154) circle (1pt);
\filldraw (3.52114417998, 45.9757963595) circle (1pt);
\filldraw (2.14410382816, 36.4800581434) circle (1pt);
\filldraw (2.55189276993, 60.9715991309) circle (1pt);
\filldraw (2.80588338969, 46.8584538547) circle (1pt);
\filldraw (2.90245948241, 59.2814487384) circle (1pt);
\filldraw (2.91971582302, 27.7752298434) circle (1pt);
\filldraw (3.54045553507, 60.8030188412) circle (1pt);
\filldraw (2.65424295239, 44.8822864909) circle (1pt);
\filldraw (3.55316057098, 80.8900242337) circle (1pt);
\filldraw (2.91511499028, 30.5349275458) circle (1pt);
\filldraw (3.32732512581, 60.7818439737) circle (1pt);
\filldraw (3.13031258211, 45.1521316739) circle (1pt);
\filldraw (3.20871215834, 27.6601494552) circle (1pt);
\filldraw (2.23984975581, 46.957661259) circle (1pt);
\filldraw (3.25168069769, 37.9188155378) circle (1pt);
\filldraw (2.89974684568, 48.7814990998) circle (1pt);
\filldraw (3.8256890776, 45.0067502997) circle (1pt);
\filldraw (3.23682278301, 62.4201670283) circle (1pt);
\filldraw (3.92853399209, 60.1933073239) circle (1pt);
\filldraw (2.89262444449, 61.0924148107) circle (1pt);
\filldraw (2.51864538702, 34.2988267055) circle (1pt);
\filldraw (3.31607704486, 53.2469690417) circle (1pt);
\filldraw (3.50537624892, 60.1737907212) circle (1pt);
\filldraw (2.74735410631, 41.5922043901) circle (1pt);
\filldraw (2.76922081749, 22.785923174) circle (1pt);
\filldraw (2.157402006, 34.0507944119) circle (1pt);
\filldraw (2.92782237247, 51.1627055724) circle (1pt);
\filldraw (2.02181383895, 10.1716131535) circle (1pt);
\filldraw (2.82431838692, 38.9321434923) circle (1pt);
\filldraw (1.84653816245, 35.4203642181) circle (1pt);
\filldraw (3.19106479257, 50.8641231134) circle (1pt);
\filldraw (2.17453489689, 22.3806408826) circle (1pt);
\filldraw (2.53573459029, 0.731642284453) circle (1pt);
\filldraw (3.35851749561, 51.205318918) circle (1pt);
\filldraw (2.97496102155, 24.7505556208) circle (1pt);
\filldraw (2.71942153331, 44.1355963595) circle (1pt);
\filldraw (2.31381755548, 36.0075629974) circle (1pt);
\filldraw (2.26876792855, 54.9227426118) circle (1pt);
\filldraw (3.05539507234, 64.9032817803) circle (1pt);
\filldraw (2.99308552961, 15.1057155948) circle (1pt);
\filldraw (3.1746101815, 53.4287627221) circle (1pt);
\filldraw (3.21119479014, 26.1221268455) circle (1pt);
\filldraw (4.0132934313, 58.1820313609) circle (1pt);
\filldraw (3.21488227676, 37.4810228834) circle (1pt);
\filldraw (2.97330203063, 19.7722523619) circle (1pt);
\filldraw (3.06202662121, 45.8555497707) circle (1pt);
\filldraw (2.73538672009, 5.73339944234) circle (1pt);
\filldraw (2.35335472434, 52.4045817156) circle (1pt);
\filldraw (3.04164239987, 50.7761675406) circle (1pt);
\filldraw (2.29477976596, 44.4222262775) circle (1pt);
\filldraw (2.12387012284, 42.1575300774) circle (1pt);
\filldraw (2.16160112439, 51.8430339519) circle (1pt);
\filldraw (2.30100862588, 35.1495393998) circle (1pt);
\filldraw (2.89637599973, 24.1415126688) circle (1pt);
\filldraw (2.61887914155, 50.5287542355) circle (1pt);
\filldraw (2.55414320729, 13.9098947361) circle (1pt);
\filldraw (3.3623696642, 45.5157078877) circle (1pt);
\filldraw (2.48912437378, 56.0914415892) circle (1pt);
\filldraw (3.27781042045, 63.7399422432) circle (1pt);
\filldraw (2.73181144779, 37.1120081269) circle (1pt);
\filldraw (3.52252679333, 35.6192471459) circle (1pt);
\filldraw (2.68183313451, 49.4774665547) circle (1pt);
\filldraw (2.56079590474, 48.4249798214) circle (1pt);
\filldraw (2.43338356017, 30.6953080244) circle (1pt);
\filldraw (2.99329834299, 25.8915417946) circle (1pt);
\filldraw (3.55583077077, 62.506197298) circle (1pt);
\filldraw (2.54143998755, 45.6960824592) circle (1pt);
\filldraw (3.03080050658, 61.8223206117) circle (1pt);
\filldraw (2.84764374411, 32.3797367079) circle (1pt);
\filldraw (3.08252574367, 54.30124633) circle (1pt);
\filldraw (2.99312743759, -2.37598280113) circle (1pt);
\filldraw (3.02461917829, 30.5738154779) circle (1pt);
\filldraw (3.29902319005, 21.2357162379) circle (1pt);
\filldraw (2.28112205287, 21.0463032378) circle (1pt);
\filldraw (3.50358160432, 71.7018892236) circle (1pt);
\filldraw (2.46664046462, 52.3208083699) circle (1pt);
\filldraw (3.2792660596, 43.9352182384) circle (1pt);
\filldraw (3.5734069816, 30.6389684662) circle (1pt);
\filldraw (3.147558292, 71.1403642784) circle (1pt);
\filldraw (2.48626458371, 36.7815519455) circle (1pt);
\filldraw (2.38600923153, 41.0930771814) circle (1pt);
\filldraw (2.93470092347, 30.4498024949) circle (1pt);
\filldraw (2.32460514053, 19.5785781028) circle (1pt);
\filldraw (2.42436988427, 41.2764272945) circle (1pt);
\filldraw (1.99848079644, 34.7185954423) circle (1pt);
\filldraw (3.8181809271, 41.203109065) circle (1pt);
\filldraw (3.21164546973, 37.198829161) circle (1pt);
\filldraw (3.51453311653, 61.3888881545) circle (1pt);
\filldraw (2.89090932861, 68.3311832807) circle (1pt);
\filldraw (2.77839963241, 49.7901216749) circle (1pt);
\filldraw (3.31642587774, 42.8681458386) circle (1pt);
\filldraw (2.56327550259, 50.9100824366) circle (1pt);
\filldraw (2.15490305821, 34.718470707) circle (1pt);
\filldraw (2.3265349552, 57.1358310957) circle (1pt);
\filldraw (2.68975099478, 45.3349538845) circle (1pt);
\filldraw (3.63496855861, 59.4135147108) circle (1pt);
\filldraw (2.42081116075, 46.202886139) circle (1pt);
\filldraw (3.29978479372, 39.89808016) circle (1pt);
\filldraw (2.90244527698, 55.8105345934) circle (1pt);
\filldraw (2.8827943808, 65.9095429431) circle (1pt);
\filldraw (3.66329162502, 33.6858545129) circle (1pt);
\filldraw (3.16545862029, 32.7654507412) circle (1pt);
\filldraw (2.30542466009, 52.5361747416) circle (1pt);
\filldraw (2.76640025672, 50.3682923712) circle (1pt);
\filldraw (3.19037453367, 66.9546682254) circle (1pt);
\filldraw (3.03900312698, 33.237598339) circle (1pt);
\filldraw (2.74259996029, 63.9774213793) circle (1pt);
\filldraw (2.22802320985, 53.5097376861) circle (1pt);
\node[anchor=center] at (1.8353666626, 37.8474861957) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-424-\imagesuffix.\imageext}};
\node[anchor=center] at (2.59706232542, 61.5330411455) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-361-\imagesuffix.\imageext}};
\node[anchor=center] at (2.25339483575, -3.98864867671) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-360-\imagesuffix.\imageext}};
\node[anchor=center] at (1.80003102238, 46.002064304) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-353-\imagesuffix.\imageext}};
\node[anchor=center] at (5.26196144276, 88.7433393301) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-327-\imagesuffix.\imageext}};
\node[anchor=center] at (3.19897276416, -7.53444286166) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-318-\imagesuffix.\imageext}};
\node[anchor=center] at (2.55817980652, 16.4313384265) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-278-\imagesuffix.\imageext}};
\node[anchor=center] at (1.77005378096, 41.2165232998) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-261-\imagesuffix.\imageext}};
\node[anchor=center] at (2.09939088309, 2.92356136148) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-260-\imagesuffix.\imageext}};
\node[anchor=center] at (4.16097711195, 42.099307114) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-243-\imagesuffix.\imageext}};
\node[anchor=center] at (2.50015389174, -17.276230832) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-232-\imagesuffix.\imageext}};
\node[anchor=center] at (3.92108468668, 68.3812157154) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-210-\imagesuffix.\imageext}};
\node[anchor=center] at (2.07336687642, -15.2368622023) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-190-\imagesuffix.\imageext}};
\node[anchor=center] at (3.82670737471, 18.8483111854) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-174-\imagesuffix.\imageext}};
\node[anchor=center] at (1.91589684645, 37.3667764851) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-151-\imagesuffix.\imageext}};
\node[anchor=center] at (2.44268144639, 49.9439026367) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-128-\imagesuffix.\imageext}};
\node[anchor=center] at (3.52946247878, 20.7362289314) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-115-\imagesuffix.\imageext}};
\node[anchor=center] at (3.99755164416, 42.343650431) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-107-\imagesuffix.\imageext}};
\node[anchor=center] at (3.01819599917, -19.2296312063) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-104-\imagesuffix.\imageext}};
\node[anchor=center] at (3.3963129242, 64.3807797132) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-103-\imagesuffix.\imageext}};
\node[anchor=center] at (4.20607296229, 82.1539161289) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-86-\imagesuffix.\imageext}};
\node[anchor=center] at (2.10616200204, 24.491145643) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-65-\imagesuffix.\imageext}};
\node[anchor=center] at (3.70627822306, 76.6481289338) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-39-\imagesuffix.\imageext}};
\node[anchor=center] at (4.54929565506, 67.6557906467) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-37-\imagesuffix.\imageext}};
\node[anchor=center] at (2.91881613935, 67.3418896109) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-14-\imagesuffix.\imageext}};
\node[anchor=center] at (3.31085967524, 55.5106176272) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-10-\imagesuffix.\imageext}};
\node[anchor=center] at (2.88819278941, 50.2471223975) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-5-\imagesuffix.\imageext}};
\node[anchor=center] at (2.53172975859, 56.4218695397) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-4-\imagesuffix.\imageext}};
\node[anchor=center] at (2.31766278875, 31.799099256) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-0-\imagesuffix.\imageext}};


==> figures/information_gains_eDN.tex <==
\filldraw (2.75628735815, 48.8573788505) circle (1pt);
\filldraw (2.24298312186, 52.9469598324) circle (1pt);
\filldraw (2.97801211785, 37.175038457) circle (1pt);
\filldraw (2.34572990786, 50.5047853311) circle (1pt);
\filldraw (2.61244411197, 44.5805927707) circle (1pt);
\filldraw (2.58626052495, 51.4878393492) circle (1pt);
\filldraw (2.46729941717, 67.3352933532) circle (1pt);
\filldraw (2.30747631695, 47.9593213983) circle (1pt);
\filldraw (3.33078763402, 58.2023000591) circle (1pt);
\filldraw (2.91484561608, 45.4464700758) circle (1pt);
\filldraw (2.60360118347, 16.8947030003) circle (1pt);
\filldraw (2.66507773942, 55.9738809543) circle (1pt);
\filldraw (2.31997095442, 53.5400337017) circle (1pt);
\filldraw (3.65515491734, 54.3835830405) circle (1pt);
\filldraw (3.0329520141, 38.6740075297) circle (1pt);
\filldraw (2.95968348844, 29.5897393323) circle (1pt);
\filldraw (2.95155992666, 54.0412318945) circle (1pt);
\filldraw (3.22235926758, 49.2485915042) circle (1pt);
\filldraw (2.46373672668, 49.5710960275) circle (1pt);
\filldraw (2.66197679004, 57.0698843678) circle (1pt);
\filldraw (2.78988300487, 41.3340617684) circle (1pt);
\filldraw (3.07605779985, 16.6695395908) circle (1pt);
\filldraw (2.41016676761, 43.1092790185) circle (1pt);
\filldraw (2.51526082509, 49.5033653162) circle (1pt);
\filldraw (3.81813052482, 73.8400623186) circle (1pt);
\filldraw (3.30915494738, 65.9628149612) circle (1pt);
\filldraw (2.33948031515, 30.8027930084) circle (1pt);
\filldraw (2.8048642717, 50.0401635488) circle (1pt);
\filldraw (2.64395860481, 33.5408313212) circle (1pt);
\filldraw (3.63572265949, 68.1484347454) circle (1pt);
\filldraw (2.457339633, 37.5109655607) circle (1pt);
\filldraw (2.92782906242, 68.7670471319) circle (1pt);
\filldraw (3.15958971312, 23.2521432804) circle (1pt);
\filldraw (2.53905930651, 31.8115632199) circle (1pt);
\filldraw (2.67685357278, 11.1673040742) circle (1pt);
\filldraw (3.17318514919, 55.1137657538) circle (1pt);
\filldraw (1.90385760345, 12.6203487555) circle (1pt);
\filldraw (3.46555938588, 64.0813472643) circle (1pt);
\filldraw (2.57801224683, 42.1761439186) circle (1pt);
\filldraw (2.2767703124, 37.3762581486) circle (1pt);
\filldraw (3.12969729221, 35.6041765995) circle (1pt);
\filldraw (2.95895927482, 25.5666712183) circle (1pt);
\filldraw (2.70467463589, 57.3822704145) circle (1pt);
\filldraw (2.80848882487, 36.7770506004) circle (1pt);
\filldraw (3.04135161212, 45.9101343055) circle (1pt);
\filldraw (2.97251555438, 50.6400067887) circle (1pt);
\filldraw (2.88106941369, 34.5785823152) circle (1pt);
\filldraw (2.24093688711, 33.2915345917) circle (1pt);
\filldraw (2.65369274586, 43.1894963244) circle (1pt);
\filldraw (2.80917533892, 46.6871808539) circle (1pt);
\filldraw (2.85036608977, 47.7440356457) circle (1pt);
\filldraw (2.45270722533, 53.4546921046) circle (1pt);
\filldraw (3.09639755938, 53.1336889235) circle (1pt);
\filldraw (2.88591605328, 51.7182014815) circle (1pt);
\filldraw (2.60982746578, 21.5828494793) circle (1pt);
\filldraw (2.21117352229, 20.3600888869) circle (1pt);
\filldraw (2.09361467566, 26.3947980485) circle (1pt);
\filldraw (2.53027408135, 64.3921641401) circle (1pt);
\filldraw (2.55499748005, 65.8728310177) circle (1pt);
\filldraw (2.95135185707, 56.8207968321) circle (1pt);
\filldraw (2.7834354129, 61.5314625838) circle (1pt);
\filldraw (2.4971459385, 64.1507450256) circle (1pt);
\filldraw (2.56999572106, 63.7692814775) circle (1pt);
\filldraw (2.87800355161, 54.0823947671) circle (1pt);
\filldraw (3.47940927804, 54.9260039959) circle (1pt);
\filldraw (2.96895017484, 27.5357076523) circle (1pt);
\filldraw (2.41327908521, 34.9585163125) circle (1pt);
\filldraw (2.56496598565, 52.6868757114) circle (1pt);
\filldraw (2.64653803204, 66.1890816463) circle (1pt);
\filldraw (3.11256125497, 62.4842720801) circle (1pt);
\filldraw (2.4912851486, 46.7777417766) circle (1pt);
\filldraw (2.85631184337, 56.5956988396) circle (1pt);
\filldraw (2.92914629726, 46.1118236681) circle (1pt);
\filldraw (2.79746594029, 66.2190412036) circle (1pt);
\filldraw (2.48143731709, 16.7129025342) circle (1pt);
\filldraw (3.9494449262, 53.5545704385) circle (1pt);
\filldraw (3.0749608549, 63.5684419139) circle (1pt);
\filldraw (3.03872454688, 44.3945245713) circle (1pt);
\filldraw (3.35075873339, 33.601534526) circle (1pt);
\filldraw (3.21927412194, 36.4894134716) circle (1pt);
\filldraw (2.70169877705, 57.1823312) circle (1pt);
\filldraw (2.62709222423, 21.8171137042) circle (1pt);
\filldraw (2.1453917887, 55.7010268641) circle (1pt);
\filldraw (2.23419042313, 48.3033391646) circle (1pt);
\filldraw (3.34322780157, 39.4091411739) circle (1pt);
\filldraw (3.72488817418, 53.8769889555) circle (1pt);
\filldraw (3.04448850223, 34.5555049333) circle (1pt);
\filldraw (3.39107048598, 40.9455250063) circle (1pt);
\filldraw (2.60316719083, 66.4854741513) circle (1pt);
\filldraw (3.1521985385, 39.5265967986) circle (1pt);
\filldraw (2.40548775918, 50.0135629198) circle (1pt);
\filldraw (2.34886881669, 42.8613029833) circle (1pt);
\filldraw (2.69636621937, 54.0854485304) circle (1pt);
\filldraw (2.47722364939, 56.8360491693) circle (1pt);
\filldraw (2.26843358119, 33.2312504221) circle (1pt);
\filldraw (2.48210412197, 62.3097253326) circle (1pt);
\filldraw (2.81407573955, 48.279530931) circle (1pt);
\filldraw (3.33659759686, 61.2432698242) circle (1pt);
\filldraw (3.49161934471, 51.3412338117) circle (1pt);
\filldraw (2.84128625467, 30.418743819) circle (1pt);
\filldraw (2.18652098541, 45.1812805894) circle (1pt);
\filldraw (2.28160163129, 28.4407310139) circle (1pt);
\filldraw (2.69800434151, 41.3910670604) circle (1pt);
\filldraw (3.19288271646, 54.8401143966) circle (1pt);
\filldraw (2.76297904171, 33.8260454727) circle (1pt);
\filldraw (2.68062227435, 53.8898046255) circle (1pt);
\filldraw (2.82153332929, 53.5491589077) circle (1pt);
\filldraw (3.11659150638, 37.086268769) circle (1pt);
\filldraw (3.13468662555, 42.794699809) circle (1pt);
\filldraw (3.54607667145, 33.5860600971) circle (1pt);
\filldraw (2.29647128477, 27.826476526) circle (1pt);
\filldraw (2.38228508563, 34.4861472525) circle (1pt);
\filldraw (3.15435965733, 21.9064081611) circle (1pt);
\filldraw (2.83774912265, 55.9315771161) circle (1pt);
\filldraw (2.81871652392, 57.8748628329) circle (1pt);
\filldraw (2.82441855463, 63.4781104546) circle (1pt);
\filldraw (2.78150939745, 23.3765846614) circle (1pt);
\filldraw (3.90084227816, 37.4546949745) circle (1pt);
\filldraw (2.76323718248, 45.6490320616) circle (1pt);
\filldraw (3.06804589243, 55.4841372588) circle (1pt);
\filldraw (3.30631134059, 48.0026095484) circle (1pt);
\filldraw (2.98492162199, 45.0567125837) circle (1pt);
\filldraw (2.75285773065, 65.7032496846) circle (1pt);
\filldraw (2.68918909611, 49.5912652492) circle (1pt);
\filldraw (4.09781856656, 63.3763258312) circle (1pt);
\filldraw (2.6180121029, 33.1356588189) circle (1pt);
\filldraw (3.77904424789, 28.9186674382) circle (1pt);
\filldraw (2.95777341877, 49.4506966237) circle (1pt);
\filldraw (2.38934020862, 47.7707647883) circle (1pt);
\filldraw (3.17122607663, 35.1518466404) circle (1pt);
\filldraw (4.17575852741, 47.1961554483) circle (1pt);
\filldraw (2.49199406207, 32.6064882551) circle (1pt);
\filldraw (2.92435861971, 35.8975148225) circle (1pt);
\filldraw (3.10809272865, 41.317096806) circle (1pt);
\filldraw (2.86020579265, 72.7318789894) circle (1pt);
\filldraw (3.26637437632, 51.8977634823) circle (1pt);
\filldraw (3.2133085336, 35.0483512971) circle (1pt);
\filldraw (2.36901958624, 44.1256332111) circle (1pt);
\filldraw (2.92052275717, 56.9178956614) circle (1pt);
\filldraw (2.77900464806, 36.3773597437) circle (1pt);
\filldraw (2.29729335467, 45.0757688665) circle (1pt);
\filldraw (2.76635762228, 9.35525069186) circle (1pt);
\filldraw (3.76452829744, 57.1269810839) circle (1pt);
\filldraw (3.05335508826, 42.3463690439) circle (1pt);
\filldraw (3.22181726739, 52.193449816) circle (1pt);
\filldraw (2.95637804486, 42.634955105) circle (1pt);
\filldraw (2.61274754154, 57.0047399013) circle (1pt);
\filldraw (2.33694479808, 31.3957403939) circle (1pt);
\filldraw (3.50821376546, 36.4406477043) circle (1pt);
\filldraw (2.324765685, 36.7162882015) circle (1pt);
\filldraw (2.5021883186, 63.6291330801) circle (1pt);
\filldraw (3.08781745451, 62.5120201708) circle (1pt);
\filldraw (2.43583394796, 65.1472685127) circle (1pt);
\filldraw (3.08916204695, 30.3939819873) circle (1pt);
\filldraw (2.55755129544, 59.0797031729) circle (1pt);
\filldraw (2.74417990566, 42.7767875684) circle (1pt);
\filldraw (2.44202478994, 9.51727704496) circle (1pt);
\filldraw (3.1795299594, 48.7304206009) circle (1pt);
\filldraw (2.32936807493, 52.6366662057) circle (1pt);
\filldraw (3.204625918, 45.4373210459) circle (1pt);
\filldraw (3.24176822975, 36.2785626135) circle (1pt);
\filldraw (2.77567353362, 14.286758818) circle (1pt);
\filldraw (2.46424967258, 11.8620815237) circle (1pt);
\filldraw (2.57849895356, 62.7802125045) circle (1pt);
\filldraw (3.53481742706, 60.0348342627) circle (1pt);
\filldraw (2.42944163452, 28.4128847821) circle (1pt);
\filldraw (2.35113463883, 56.4501294452) circle (1pt);
\filldraw (3.86309982107, 50.6787459532) circle (1pt);
\filldraw (3.71369348777, 50.8716531898) circle (1pt);
\filldraw (2.63934227042, 62.9671076383) circle (1pt);
\filldraw (2.702170052, 0.928567988542) circle (1pt);
\filldraw (2.76545639724, 39.1889565225) circle (1pt);
\filldraw (3.33962827315, 31.6934443151) circle (1pt);
\filldraw (2.92544900927, 64.4313544388) circle (1pt);
\filldraw (2.39583582869, 23.5093909752) circle (1pt);
\filldraw (2.74174749, 68.9132219083) circle (1pt);
\filldraw (2.69296637046, 42.2885449285) circle (1pt);
\filldraw (3.0855296822, 69.4713908829) circle (1pt);
\filldraw (2.11591504049, 24.7112592734) circle (1pt);
\filldraw (3.14852808913, 45.2861693027) circle (1pt);
\filldraw (2.79445584341, 46.4701140225) circle (1pt);
\filldraw (2.79599905623, 55.3404503822) circle (1pt);
\filldraw (1.85726770026, 39.06885335) circle (1pt);
\filldraw (2.69981616984, 48.0963443477) circle (1pt);
\filldraw (2.25890958952, 26.4942138534) circle (1pt);
\filldraw (2.2669950975, 26.7491649527) circle (1pt);
\filldraw (3.15540188569, 39.7904415412) circle (1pt);
\filldraw (2.50188485039, 45.3751091022) circle (1pt);
\filldraw (3.44037931922, 54.6190238211) circle (1pt);
\filldraw (2.92390830976, 52.6275796343) circle (1pt);
\filldraw (3.11674458299, 35.9169966647) circle (1pt);
\filldraw (2.36098134693, 50.546753732) circle (1pt);
\filldraw (3.39673105057, 50.8968960264) circle (1pt);
\filldraw (2.79249615531, 35.7293667176) circle (1pt);
\filldraw (2.63144322244, 38.4820359031) circle (1pt);
\filldraw (2.79443179581, 38.5720596416) circle (1pt);
\filldraw (2.56705273233, 54.7342600266) circle (1pt);
\filldraw (2.6916933733, 48.565913711) circle (1pt);
\filldraw (2.86363739968, 54.3930035397) circle (1pt);
\filldraw (2.80006180504, 50.181877857) circle (1pt);
\filldraw (3.04818473348, 44.2664001318) circle (1pt);
\filldraw (2.77699908715, 55.7577144394) circle (1pt);
\filldraw (3.8015607397, 28.0883341897) circle (1pt);
\filldraw (2.48281194638, 30.1572624827) circle (1pt);
\filldraw (2.65659881831, 30.5133514813) circle (1pt);
\filldraw (2.30168222691, 40.7550570686) circle (1pt);
\filldraw (2.43436823546, 52.125852087) circle (1pt);
\filldraw (2.25662724973, 20.413497732) circle (1pt);
\filldraw (2.57887876166, 19.0176211013) circle (1pt);
\filldraw (2.71654738539, 51.5740226595) circle (1pt);
\filldraw (3.06319590806, 54.6152104869) circle (1pt);
\filldraw (2.19869388505, 38.0620874425) circle (1pt);
\filldraw (3.55555396812, 55.2836987044) circle (1pt);
\filldraw (3.11704792023, 65.2041613871) circle (1pt);
\filldraw (3.2352143723, 61.1835125526) circle (1pt);
\filldraw (2.15334701869, 38.1639094048) circle (1pt);
\filldraw (2.79650190679, 46.46814488) circle (1pt);
\filldraw (2.76732034248, 55.0931919393) circle (1pt);
\filldraw (2.86662875205, 56.675501172) circle (1pt);
\filldraw (3.09855643238, 16.6056348664) circle (1pt);
\filldraw (3.35362812086, 68.7013734616) circle (1pt);
\filldraw (3.30158312847, 58.610774508) circle (1pt);
\filldraw (2.41234898302, 62.2401782203) circle (1pt);
\filldraw (3.04933414907, 43.8625912886) circle (1pt);
\filldraw (3.1514403271, 40.8553912587) circle (1pt);
\filldraw (2.49876679641, 40.4708381995) circle (1pt);
\filldraw (3.04317580738, 22.2733879057) circle (1pt);
\filldraw (3.98942212466, 56.316392059) circle (1pt);
\filldraw (2.67003144792, 13.0067401777) circle (1pt);
\filldraw (2.57219326496, 32.3667035069) circle (1pt);
\filldraw (3.10064490939, 65.1442794148) circle (1pt);
\filldraw (2.89130020701, 30.7863957277) circle (1pt);
\filldraw (4.21482792059, 59.9680746642) circle (1pt);
\filldraw (2.98808396391, 55.3229909682) circle (1pt);
\filldraw (2.8667541359, 36.4067571812) circle (1pt);
\filldraw (2.38897425327, 53.3741691284) circle (1pt);
\filldraw (3.55701301457, 62.6264682767) circle (1pt);
\filldraw (2.90372417752, 45.358772083) circle (1pt);
\filldraw (3.24352323956, 56.120553217) circle (1pt);
\filldraw (3.0794856707, 40.977776501) circle (1pt);
\filldraw (2.90682756203, 44.7024100442) circle (1pt);
\filldraw (2.6584328992, 36.191310293) circle (1pt);
\filldraw (3.02438462868, 71.6555815846) circle (1pt);
\filldraw (2.29298655025, 54.0682931661) circle (1pt);
\filldraw (2.68213757045, 27.8225291769) circle (1pt);
\filldraw (3.45742828884, 64.2612923667) circle (1pt);
\filldraw (3.4943148838, 17.1825545862) circle (1pt);
\filldraw (3.41681721143, 40.5858098132) circle (1pt);
\filldraw (2.51380355887, 41.604542149) circle (1pt);
\filldraw (2.84805957288, 51.7786338377) circle (1pt);
\filldraw (1.9923127202, 54.9749014646) circle (1pt);
\filldraw (2.81408542949, 27.0889442999) circle (1pt);
\filldraw (2.89517648226, 5.78530667074) circle (1pt);
\filldraw (3.07466586169, 57.9530213688) circle (1pt);
\filldraw (2.53002213323, 37.5432784249) circle (1pt);
\filldraw (2.7127547372, 60.1127177459) circle (1pt);
\filldraw (2.53320257013, 19.5937327719) circle (1pt);
\filldraw (2.24148953834, 13.5013823493) circle (1pt);
\filldraw (2.31539909856, 37.1070461859) circle (1pt);
\filldraw (2.2689990907, 49.707195317) circle (1pt);
\filldraw (2.63574670666, 56.036020826) circle (1pt);
\filldraw (3.46587805049, 64.4869277712) circle (1pt);
\filldraw (3.00742348204, 48.0818154673) circle (1pt);
\filldraw (3.69600466214, 61.4816993602) circle (1pt);
\filldraw (2.8779700098, 15.5836593207) circle (1pt);
\filldraw (2.48161775132, 54.8790571685) circle (1pt);
\filldraw (2.13691668521, 48.0385636076) circle (1pt);
\filldraw (1.85360670891, 34.6487358127) circle (1pt);
\filldraw (3.02445201106, 67.3045505882) circle (1pt);
\filldraw (2.84908920095, 57.789712406) circle (1pt);
\filldraw (3.54775233476, 33.7576845441) circle (1pt);
\filldraw (3.71148900205, 63.7764493637) circle (1pt);
\filldraw (2.92452587279, 65.8384319093) circle (1pt);
\filldraw (2.67757696734, 10.322973171) circle (1pt);
\filldraw (2.04051854342, 35.3826247424) circle (1pt);
\filldraw (3.231479136, 71.5984285069) circle (1pt);
\filldraw (2.68650596684, 56.6178136871) circle (1pt);
\filldraw (3.29891944332, 65.4723702257) circle (1pt);
\filldraw (2.79971815649, 30.150713693) circle (1pt);
\filldraw (2.96533058946, 49.4551357488) circle (1pt);
\filldraw (2.54957640485, 57.4549530113) circle (1pt);
\filldraw (2.70499912965, 51.2044127325) circle (1pt);
\filldraw (2.50093315963, 49.6843454766) circle (1pt);
\filldraw (3.06235061038, 67.8032500193) circle (1pt);
\filldraw (1.96131531408, 18.1392581523) circle (1pt);
\filldraw (2.79866322861, 5.54499483489) circle (1pt);
\filldraw (2.63714362481, 32.549284221) circle (1pt);
\filldraw (3.28693598115, 58.6957496621) circle (1pt);
\filldraw (3.90878239968, 58.1141138237) circle (1pt);
\filldraw (2.76491782628, 61.458697655) circle (1pt);
\filldraw (2.50879054867, 43.8273193472) circle (1pt);
\filldraw (2.31029140575, 44.6192787123) circle (1pt);
\filldraw (3.20079429964, 52.2946248533) circle (1pt);
\filldraw (3.57633033988, 48.1022029158) circle (1pt);
\filldraw (2.29268959165, 43.897535707) circle (1pt);
\filldraw (2.94967417629, 48.8083740947) circle (1pt);
\filldraw (3.00894124182, 30.5296597943) circle (1pt);
\filldraw (2.73384957096, 34.4504294674) circle (1pt);
\filldraw (1.97096492885, 27.8951892918) circle (1pt);
\filldraw (3.01912063727, 61.1545036537) circle (1pt);
\filldraw (2.33943210156, 50.76194355) circle (1pt);
\filldraw (2.83421691085, 25.7336463565) circle (1pt);
\filldraw (2.37405008767, 7.04231993975) circle (1pt);
\filldraw (3.84481353269, 52.4699604094) circle (1pt);
\filldraw (3.24120424267, 51.2007017125) circle (1pt);
\filldraw (2.61527779345, 7.63327356803) circle (1pt);
\filldraw (2.61885074379, 53.6583978163) circle (1pt);
\filldraw (2.83347546389, 40.6124665509) circle (1pt);
\filldraw (2.59875621755, 45.9981399448) circle (1pt);
\filldraw (2.41199812649, 56.0554840861) circle (1pt);
\filldraw (2.27786707343, 48.2256191051) circle (1pt);
\filldraw (2.75118687756, 59.7807007169) circle (1pt);
\filldraw (2.35543509058, 44.568997807) circle (1pt);
\filldraw (3.23648097861, 55.1539409715) circle (1pt);
\filldraw (2.40787106924, 50.3772077765) circle (1pt);
\filldraw (2.06017594745, 25.5951352569) circle (1pt);
\filldraw (3.62416199961, 73.7926622396) circle (1pt);
\filldraw (2.9873891576, 49.8131341962) circle (1pt);
\filldraw (2.29672095846, 41.8402090044) circle (1pt);
\filldraw (2.14627504496, 51.5430406361) circle (1pt);
\filldraw (3.39428630244, 44.2907860148) circle (1pt);
\filldraw (3.28408801105, 25.353735311) circle (1pt);
\filldraw (4.02850252866, 58.0746913828) circle (1pt);
\filldraw (2.66156506891, 22.3573505878) circle (1pt);
\filldraw (3.69840764902, 54.596692253) circle (1pt);
\filldraw (2.94640229489, 58.9536960266) circle (1pt);
\filldraw (3.52114417998, 44.9782705605) circle (1pt);
\filldraw (2.14410382816, 19.4819402846) circle (1pt);
\filldraw (2.55189276993, 60.7996819205) circle (1pt);
\filldraw (2.80588338969, 51.9078264711) circle (1pt);
\filldraw (2.90245948241, 64.4060031489) circle (1pt);
\filldraw (2.91971582302, 31.6672345727) circle (1pt);
\filldraw (3.54045553507, 61.5795157234) circle (1pt);
\filldraw (2.65424295239, 39.4216879992) circle (1pt);
\filldraw (3.55316057098, 73.3383252255) circle (1pt);
\filldraw (2.91511499028, 23.8543419355) circle (1pt);
\filldraw (3.32732512581, 59.2729466466) circle (1pt);
\filldraw (3.13031258211, 42.9343739698) circle (1pt);
\filldraw (3.20871215834, 45.8726590699) circle (1pt);
\filldraw (2.23984975581, 33.7755615831) circle (1pt);
\filldraw (3.25168069769, 49.8228101563) circle (1pt);
\filldraw (2.89974684568, 60.7981882913) circle (1pt);
\filldraw (3.8256890776, 62.144562928) circle (1pt);
\filldraw (3.23682278301, 64.5360525734) circle (1pt);
\filldraw (3.92853399209, 67.4769726147) circle (1pt);
\filldraw (2.89262444449, 60.8686072611) circle (1pt);
\filldraw (2.51864538702, 39.9146542059) circle (1pt);
\filldraw (3.31607704486, 69.6779378501) circle (1pt);
\filldraw (3.50537624892, 71.1937591687) circle (1pt);
\filldraw (2.74735410631, 49.7967777577) circle (1pt);
\filldraw (2.76922081749, 15.6553041721) circle (1pt);
\filldraw (2.157402006, 37.7972938469) circle (1pt);
\filldraw (2.92782237247, 51.7867555601) circle (1pt);
\filldraw (2.02181383895, 18.0082725119) circle (1pt);
\filldraw (2.82431838692, 50.3317883043) circle (1pt);
\filldraw (1.84653816245, 26.8050463449) circle (1pt);
\filldraw (3.19106479257, 47.3370753018) circle (1pt);
\filldraw (2.17453489689, 30.5678438356) circle (1pt);
\filldraw (2.53573459029, 28.783317716) circle (1pt);
\filldraw (3.35851749561, 52.039130444) circle (1pt);
\filldraw (2.97496102155, 40.8797978896) circle (1pt);
\filldraw (2.71942153331, 55.1881391756) circle (1pt);
\filldraw (2.31381755548, 50.9464958627) circle (1pt);
\filldraw (2.26876792855, 53.1967161658) circle (1pt);
\filldraw (3.05539507234, 60.5046117072) circle (1pt);
\filldraw (2.99308552961, 13.2937969947) circle (1pt);
\filldraw (3.1746101815, 56.0195940693) circle (1pt);
\filldraw (3.21119479014, 46.4718538573) circle (1pt);
\filldraw (4.0132934313, 60.1472888146) circle (1pt);
\filldraw (3.21488227676, 57.3935729727) circle (1pt);
\filldraw (2.97330203063, 21.3642607376) circle (1pt);
\filldraw (3.06202662121, 46.5793147899) circle (1pt);
\filldraw (2.73538672009, 36.8371068279) circle (1pt);
\filldraw (2.35335472434, 47.5263255052) circle (1pt);
\filldraw (3.04164239987, 43.0395294697) circle (1pt);
\filldraw (2.29477976596, 48.9246802272) circle (1pt);
\filldraw (2.12387012284, 32.9940790556) circle (1pt);
\filldraw (2.16160112439, 53.3485160249) circle (1pt);
\filldraw (2.30100862588, 35.8496848157) circle (1pt);
\filldraw (2.89637599973, 22.7251874636) circle (1pt);
\filldraw (2.61887914155, 59.4038162286) circle (1pt);
\filldraw (2.55414320729, 46.9085908556) circle (1pt);
\filldraw (3.3623696642, 45.0609408532) circle (1pt);
\filldraw (2.48912437378, 48.5259913601) circle (1pt);
\filldraw (3.27781042045, 47.4022706723) circle (1pt);
\filldraw (2.73181144779, 53.3035459604) circle (1pt);
\filldraw (3.52252679333, 42.9657132272) circle (1pt);
\filldraw (2.68183313451, 46.8086206403) circle (1pt);
\filldraw (2.56079590474, 51.9842527089) circle (1pt);
\filldraw (2.43338356017, 53.8440665661) circle (1pt);
\filldraw (2.99329834299, 32.4715916008) circle (1pt);
\filldraw (3.55583077077, 70.3238134689) circle (1pt);
\filldraw (2.54143998755, 55.4722457077) circle (1pt);
\filldraw (3.03080050658, 45.6288115656) circle (1pt);
\filldraw (2.84764374411, 44.7014922513) circle (1pt);
\filldraw (3.08252574367, 71.1033401684) circle (1pt);
\filldraw (2.99312743759, 20.6628804861) circle (1pt);
\filldraw (3.02461917829, 36.0270888832) circle (1pt);
\filldraw (3.29902319005, 42.9821076876) circle (1pt);
\filldraw (2.28112205287, 31.4769093106) circle (1pt);
\filldraw (3.50358160432, 75.3963880881) circle (1pt);
\filldraw (2.46664046462, 58.5765433868) circle (1pt);
\filldraw (3.2792660596, 49.4766802618) circle (1pt);
\filldraw (3.5734069816, 59.2718593497) circle (1pt);
\filldraw (3.147558292, 61.3372818468) circle (1pt);
\filldraw (2.48626458371, 51.1514158686) circle (1pt);
\filldraw (2.38600923153, 47.4813384758) circle (1pt);
\filldraw (2.93470092347, 43.0669118331) circle (1pt);
\filldraw (2.32460514053, 31.4702628394) circle (1pt);
\filldraw (2.42436988427, 41.4917344084) circle (1pt);
\filldraw (1.99848079644, 41.8290479883) circle (1pt);
\filldraw (3.8181809271, 50.6216168559) circle (1pt);
\filldraw (3.21164546973, 27.721389452) circle (1pt);
\filldraw (3.51453311653, 68.1587194581) circle (1pt);
\filldraw (2.89090932861, 66.0973930627) circle (1pt);
\filldraw (2.77839963241, 43.732002064) circle (1pt);
\filldraw (3.31642587774, 38.3835599712) circle (1pt);
\filldraw (2.56327550259, 38.3801208995) circle (1pt);
\filldraw (2.15490305821, 47.8709463452) circle (1pt);
\filldraw (2.3265349552, 54.6228072829) circle (1pt);
\filldraw (2.68975099478, 46.0798930306) circle (1pt);
\filldraw (3.63496855861, 75.6925684136) circle (1pt);
\filldraw (2.42081116075, 45.6734283072) circle (1pt);
\filldraw (3.29978479372, 43.8101682011) circle (1pt);
\filldraw (2.90244527698, 55.7495336412) circle (1pt);
\filldraw (2.8827943808, 70.3114203958) circle (1pt);
\filldraw (3.66329162502, 46.1306416375) circle (1pt);
\filldraw (3.16545862029, 37.3471024029) circle (1pt);
\filldraw (2.30542466009, 60.902429135) circle (1pt);
\filldraw (2.76640025672, 57.1799207505) circle (1pt);
\filldraw (3.19037453367, 60.209702653) circle (1pt);
\filldraw (3.03900312698, 47.2435952623) circle (1pt);
\filldraw (2.74259996029, 69.4541735354) circle (1pt);
\filldraw (2.22802320985, 52.2807114336) circle (1pt);
\node[anchor=center] at (1.8353666626, 27.782516397) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-424-\imagesuffix.\imageext}};
\node[anchor=center] at (2.59706232542, 73.632615538) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-361-\imagesuffix.\imageext}};
\node[anchor=center] at (2.25339483575, -13.4319659131) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-360-\imagesuffix.\imageext}};
\node[anchor=center] at (1.80003102238, 47.2267642987) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-353-\imagesuffix.\imageext}};
\node[anchor=center] at (5.26196144276, 66.1390326526) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-327-\imagesuffix.\imageext}};
\node[anchor=center] at (3.19897276416, -19.2050523905) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-318-\imagesuffix.\imageext}};
\node[anchor=center] at (2.55817980652, -0.996517071338) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-278-\imagesuffix.\imageext}};
\node[anchor=center] at (1.77005378096, 38.8781057817) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-261-\imagesuffix.\imageext}};
\node[anchor=center] at (2.09939088309, -33.0966756306) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-260-\imagesuffix.\imageext}};
\node[anchor=center] at (4.16097711195, 25.6274307554) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-243-\imagesuffix.\imageext}};
\node[anchor=center] at (2.50015389174, 26.2322701122) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-232-\imagesuffix.\imageext}};
\node[anchor=center] at (3.92108468668, 79.5385949586) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-210-\imagesuffix.\imageext}};
\node[anchor=center] at (2.07336687642, 1.30580858494) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-190-\imagesuffix.\imageext}};
\node[anchor=center] at (3.82670737471, 38.6684059563) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-174-\imagesuffix.\imageext}};
\node[anchor=center] at (1.91589684645, 54.0971628897) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-151-\imagesuffix.\imageext}};
\node[anchor=center] at (2.44268144639, 14.0660463949) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-128-\imagesuffix.\imageext}};
\node[anchor=center] at (3.52946247878, 24.5465765588) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-115-\imagesuffix.\imageext}};
\node[anchor=center] at (3.99755164416, 49.8070142566) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-107-\imagesuffix.\imageext}};
\node[anchor=center] at (3.01819599917, -7.91787306008) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-104-\imagesuffix.\imageext}};
\node[anchor=center] at (3.3963129242, 78.1561920668) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-103-\imagesuffix.\imageext}};
\node[anchor=center] at (4.20607296229, 65.7609623739) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-86-\imagesuffix.\imageext}};
\node[anchor=center] at (2.10616200204, 19.6674171113) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-65-\imagesuffix.\imageext}};
\node[anchor=center] at (3.70627822306, 58.3489037053) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-39-\imagesuffix.\imageext}};
\node[anchor=center] at (4.54929565506, 52.8298213665) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-37-\imagesuffix.\imageext}};
\node[anchor=center] at (2.91881613935, 68.6462403173) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-14-\imagesuffix.\imageext}};
\node[anchor=center] at (3.31085967524, 58.0206097863) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-10-\imagesuffix.\imageext}};
\node[anchor=center] at (2.88819278941, 56.8875169124) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-5-\imagesuffix.\imageext}};
\node[anchor=center] at (2.53172975859, 54.8143051261) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-4-\imagesuffix.\imageext}};
\node[anchor=center] at (2.31766278875, 39.6272063277) {\includegraphics[width=\pwidth\tikzunit]{information_gains/dataset/\imageprefix-0-\imagesuffix.\imageext}};


==> figures/information_gains_scatter_all.pgf.tex <==
\ifdefined\noktikz
  \input{figures/informationgainsdata}
\else
  \usetikzlibrary{calc}
  \usetikzlibrary{shapes}
  \graphicspath{{/kyb/agmb/mkuemmerer/Documents/Uni/Bethge/Saliency/presentations/poster_Bernstein_2014/figures/}}

  \input{/kyb/agmb/mkuemmerer/Documents/Uni/Bethge/Saliency/presentations/poster_Bernstein_2014/figures/informationgainsscatterdata}
\fi


\newcommand\loglik[1]{\textsf{$\mathsf{#1}$\,bits/fix}}
\newcommand\auc[1]{\textsf{$\mathsf{#1}$\,\%}}

%\newlength\imgwidth
%\setlength\imgwidth{4cm}

\ifdefined\abstikzunit
\else
	\newlength\abstikzunit
	\newlength\tikzunit
\fi

\setlength\abstikzunit{1cm}
\newcommand\scalingfactor{1.15}
\newcommand\imgwidth{5.0}
\newcommand\pwidth{0.5}
\setlength\tikzunit{\scalingfactor\abstikzunit}


\setlength\abstikzunit{1cm}
\setlength\tikzunit{\scalingfactor\abstikzunit}

%\newcommand\imgwidth{5cm}
%\newcommand\imgwidth{4cm}

% TODO:
% - colorbar, probably per image and with values

\ifdefined\noktikz
\else
  \newcommand\imageprefix{general}
  \newcommand\imagesuffix{image}
  \newcommand\imageext{png}
  \newcommand\modelname{eDN}
\fi

\begin{tikzpicture}[x=1.3*\tikzunit,y=0.03*\tikzunit,font=\small\sffamily,every node/.style={inner sep=0,outer sep=0}]
  \coordinate (xstart)  at (1.5,0);
  \coordinate (rightend) at (5.5,0);
  \coordinate (width) at ($ (rightend) - (xstart) $);
  \coordinate (height) at (0,100);
  \coordinate (height2) at (0,-50);
  \coordinate (O) at (0, 0);
  \coordinate (xticksize) at (0, -3);

  \draw[line width=0.5,dotted] ($ (xstart) + (height) $) -- ($ (rightend) + (height) $);
  \draw[line width=0.5,dotted] ($ (xstart) + (O) $) -- ($ (rightend) + (O) $);


  \ifdefined\noktikz
    \input{figures/information_gains_\modelname}
  \else
    \input{/kyb/agmb/mkuemmerer/Documents/Uni/Bethge/Saliency/presentations/poster_Bernstein_2014/figures/information_gains_\modelname}
  \fi

  \draw[line width=0.5] ($ (xstart) + (height) $)-- ($ (xstart) + (height2) $);
  \draw[line width=0.5] ($ (xstart) + (height2) $) -- ($ (xstart) + (height2) + (width) $);

  \node[anchor=north, outer sep = 5] at ($ (height2) + 0.5*(width) + (xstart) $) {\tiny Gold [bit/fix]};
  \node[anchor=south, outer sep = 5,rotate=90] at ($ (xstart) + 0.5*(height) $) {\tiny explained information};

  \foreach \xtick in {2.0,5.0}
  {
    \draw[line width=0.5] ($ (\xtick, 0) + (height2) $) -- ($ (\xtick, 0) + (height2) - (xticksize) $);
    \node[anchor=north, outer sep=5] at ($ (\xtick, 0) + (height2) $) {\tiny\xtick};
  }

  \foreach \ytick in {0,100}
  {
%    \draw[line width=1] ($ (0, \ytick) + (ticksize) $) -- ($ (\xtick, 0) + (height) - (ticksize) $);
    \node[anchor=east, outer sep=3] at ($ (0, \ytick) + (xstart) $) {\tiny\ytick \%};
  }


\end{tikzpicture}

% Clean up
\let\abstikzunit\undef
\let\scalingfactor\undef
\let\imgwidth\undef
\let\pwidth\undef
\let\tikzunit\undef


==> figures/informationgainsdata.tex <==
\expandafter\xdef\csname informationgain260BMSig\endcsname{-0.40}
\expandafter\xdef\csname informationgain210BMSig\endcsname{2.59}
\expandafter\xdef\csname informationgain163goldig\endcsname{2.80}
\expandafter\xdef\csname informationgain210AIMig\endcsname{2.28}
\expandafter\xdef\csname informationgain163eDNig\endcsname{0.16}
\expandafter\xdef\csname informationgain163AIMig\endcsname{-1.06}
\expandafter\xdef\csname informationgain260eDNig\endcsname{-0.69}
\expandafter\xdef\csname informationgain210eDNig\endcsname{3.12}
\expandafter\xdef\csname informationgain163BMSig\endcsname{-0.92}
\expandafter\xdef\csname informationgain260AIMig\endcsname{-0.59}
\expandafter\xdef\csname informationgain210goldig\endcsname{3.92}
\expandafter\xdef\csname informationgain260goldig\endcsname{2.10}
\expandafter\xdef\csname imgindexa\endcsname{210}
\expandafter\xdef\csname imgindexb\endcsname{260}
\expandafter\xdef\csname imgindexc\endcsname{163}


==> figures/model_colors.tex <==
\definecolor{colornonlinearity}{rgb}{0.98046875, 0.6015625, 0.59765625}
\definecolor{colorcenterbias}{rgb}{0.19921875, 0.625, 0.171875}
\definecolor{colorblur}{rgb}{0.6953125, 0.87109375, 0.5390625}
\definecolor{colorexcitation}{rgb}{0.12109375, 0.46875, 0.703125}
\definecolor{colorexcentric}{rgb}{0.6484375, 0.8046875, 0.88671875}

